The Sunyaev-Zel'dovich Array: Constraining a new pressure profile for fitting SZE observations of galaxy clusters

The Sunyaev-Zel'dovich Array (SZA), an eight element interferometer designed to probe the Sunyaev-Zel'dovich effect (SZE) from galaxy clusters, which I helped construct and operate, is described here (Part I). I then use SZA observations to investigate the utility of a new, self-similar pressure profile for fitting SZE observations of galaxy clusters (Part II). The SZA 30-GHz receiver system probes angular scales ~1-5'. A model that can accurately describe a cluster's pressure profile over a correspondingly broad range of radii is therefore required. In the analysis presented here, I fit a 2-parameter, radial pressure profile, derived from simulations and detailed X- ray analysis of relaxed clusters, to SZA observations of three clusters with exceptionally high quality X-ray data. From the joint analysis of the SZE and X-ray data, I derive physical properties of the cluster, such as gas and total mass, gas fraction and the integrated Compton y -parameter. The parameters derived from the joint fit to SZE+X-ray data agree well with a detailed, independent, X-ray-only analysis of these same clusters. When combined with X-ray imaging data, this new pressure profile yields an independent estimate of the electron temperature profile that is in good agreement with spectroscopic X-ray determinations. In addition to yielding relationships between cluster observables and physical cluster properties, this model could prove to be a useful tool in helping to constrain the temperatures of high redshift clusters, for which X-ray spectroscopic data are difficult to obtain.

==> app1.tex <==
\chapter{Appendix: $\delta T(R)$ from the Generalized NFW Model}

We present some useful relations for applying the generalized NFW model to fit
the underlying cluster pressure profile observed through the SZ effect.

\begin{equation}
P_e(r) = \frac{P_{e,0}}{(r/r_p)^c \left[1+(r/r_p)^a\right]^{(b-c)/a}}
\label{eq:press_append}
\end{equation}

The line-of-sight integral to compute Compton $y$ at arbitrary radius $R$ on the 
sky is:

\begin{equation}
y(R) = \frac{\sigma_T}{m_e c^2} \int_{-\infty}^\infty P_e(\sqrt{R^2+r^2})) dr.
\end{equation}

%Using the substitution $x=r/r_p$ is generally easier to implement in code, 
Using the substitution $\hat{r}=r/r_p$ is generally easier to implement in code, 
since it produces a projected profile that can be scaled according the $r_p$.
The projected profile therefore only has to be numerically integrated once (if 
the only parameters being varied are $r_p$ and $\Delta T_0$), which saves some 
computation time in a markov chain hundreds of thousands of iterations long.

%The integral becomes, for dimensionless radius $x = r/r_p$ and dimensionless 
%impact parameter $X=R/r_p$, 
The integral becomes, for dimensionless radius $\hat{r} = r/r_p$ and dimensionless 
impact parameter $\hat{R}=R/r_p$, 

%\begin{equation}
%y(R) = \frac{\sigma_T}{m_e c^2}~r_p~\int_{-\infty}^\infty P_e(\sqrt{X^2+x^2}) dx
%\end{equation}
\begin{equation}
y(R) = \frac{\sigma_T}{m_e c^2}~r_p~\int_{-\infty}^\infty P_e\left(\sqrt{\hat{R}^2+\hat{r}^2}\right) d\hat{r}
\end{equation}

The $\beta$-model has a finite value at zero
radius, so it is natural to normalize the profile to 
produce a central decrement.  This is especially convenient since the rest of 
the profile is analytically integrable.

In contrast, the generalized NFW profile is singular at the core, and has no 
analytic solution to its line-of-sight integral, so it is more natural to solve
for the projection on the sky and find the relation between the pressure 
normalization $P_{e,0}$ and the SZE normalization $\Delta T_0$ (which is not the 
central decrement, but just a scaling to the amplitude).

%For any arbitrary radius on the sky $R$, using $\Delta T(R) = f(x_{f})~y(R)~T_{cmb}$ 
%(where we have redefined dimensionless frequency as $x_{f}$ in order to 
For any arbitrary radius on the sky $R$, using $\Delta T(R) = f(\hat{\nu})~y(R)~T_{cmb}$ 
(where we have defined dimensionless frequency as $\hat{\nu}$),

%\begin{equation}
%\Delta T(R) 
%= \left[\frac{f(x_{f})~T_{cmb}~\sigma_T~r_p~P_{e,0}}{m_e c^2}\right]~
%2 \int_0^\infty
%\frac{ P_e\left(\sqrt{X^2+x^2}\right)}{P_{e,0}} dx
%\end{equation}
\begin{equation}
\Delta T(R) 
= \left[\frac{f(x_{f})~T_{cmb}~\sigma_T~r_p~P_{e,0}}{m_e c^2}\right]~
2 \int_0^\infty
\frac{ P_e\left(\sqrt{\hat{R}^2+\hat{r}^2}\right)}{P_{e,0}} d\hat{r}
\end{equation}

At some specific value of $R$, $\Delta T(R) = \Delta T_0$.  This is where the integral 
integrates to one

%\begin{equation}
%1 = 2 \int_{0}^\infty \frac{P_e(\sqrt{X^2+x^2})}{P_{e,0}} dx .
%\end{equation}
\begin{equation}
1 = 2 \int_{0}^\infty \frac{P_e\left(\sqrt{\hat{R}^2+\hat{r}^2}\right)}{P_{e,0}} d\hat{r} .
\end{equation}

So we have:

%\begin{equation}
%P_{e,0} = \frac{\Delta T_0 m_e c^2}{\sigma_T r_p f(x_{f}) T_{cmb}}
%\end{equation}
\begin{equation}
P_{e,0} = \frac{\Delta T_0 m_e c^2}{\sigma_T r_p f(\hat{\nu}) T_{cmb}}
\end{equation}



==> mockobs.tex <==
\section{Mock SZA Observations of Simulated Clusters}

We performed mock, radio-interferometric observations using {\em simint}, 
a program written by Erik Leitch, which is capable of simulating interferometric
observations (see e.g., \cite{holder2000}).  
{\em simint} Fourier transforms an astronomical image -- in this case an SZ map 
from a simulated cluster -- then samples the transform according to the baselines
and antenna apertures for the specified interferometer parameters,
injecting noise in {\em u,v}-space appropriate to the observation parameters. {\em
simint} simulates two types of noise: atmospheric, using a
user-specified opacity at zenith and an atmospheric model appropriate
for 30 GHz observations, and instrumental noise, included as a lump
temperature term meant to account for ground spillover, receiver
noise, and any other possible source of noise in the signal
chain. {\em simint} also accounts for the antenna aperature and the
correlator efficiencies.  The output of {\em simint} is a UVFITS file,
which contains observation parameters such as antenna size and spacing, 
frequency at which objects are observed, information about the target
observed, and the data points and their weights in {\em u,v}-space.

We used typical parameters for the SZA in all our mock observations. 
The atmospheric opacity at zenith was set to $\tau=0.04$ (typical of a
clear day), and the instrumental noise temperature was set to 25 K.  
The aperture efficiency was set to 0.70, and the correlator
efficiency was set to 0.87, appropriate for a digital correlator.

To perform these mock observations, we first converted the SZ
decrement maps from the numerical simulations 
to FITS format images.  During this conversion, each cluster
temperature map, which is in comoving distance units, was scaled such 
that its angular pixel size corresponded to the redshift of observation, 
using the angular diameter distance appropriate to a \LCDM\ ``concordance cosmology''
($\Omega_{\rm M}=0.3$, $\Omega_\Lambda=0.7$, $h=0.7$, consistent with the
assumed cosmology of the cluster simulations).  
These FITS images were then read into simint for the
desired track length and number of days of observation. 

We performed two types of simulated observations: one set with six
hour tracks repeated for five days of observations, which represent
realistic observations, and the other set with twelve hour tracks
repeated for one thousand days, used to calibrate the fits to the
cluster pressure profile.  The twelve hour tracks, while impossibly
long since we never observe below a 30$^\circ$ horizon, served to
optimize UV coverage when calibrating the pressure profile, while the
track repetition eliminated any confusion due to noise.  For both
types of observation, each cluster was placed at a declination of 37$^\circ$,
so that it passed through zenith. Hence the observations used for
calibration were only limited by the cluster redshift, the layout of
the SZA (which is currently fixed), and by the use of only the 30~GHz
receivers (90~GHz observations will soon be feasible as well).  The
more realistic, 30 hour observations were used to diagnose the actual
performance attainable by the SZA.



==> polytropic_model.tex <==
\subsection{Polytropic Models \label{polytropic_model}}

The assumption of isothermality does not remain valid over a broad radial extent of a cluster,
even when the core is excluded.  Early joint SZE+X-ray data fitting only allowed the SZE data
to constrain one unique parameter -- $y_0$ -- to within $\sim 10\%$ error bars.  
Since the SZA can integrate to the OVRO/BIMA signal levels
$\sim 8$ times more quickly, the resulting higher quality data of a typical 30-GHz SZA observation allows 
two parameters to be uniquely determined by SZE data.  An additional benefit of the SZA over
OVRO/BIMA is in the shorter baselines, due to the close-packed inner array (discussed in 
\S \ref{sza_overview}).  These baselines allow us to probe larger scales, where isothermality
is not expected to hold.

Early attempts at using X-ray data to move beyond the isothermal $\beta$-model
\citep[see][]{markevitch1998} utilized polytropic temperature profiles.  
A polytropic equation of state simply relates pressure to density:
\begin{equation}
P_e(r) = P_{e,0} \left[n_e(r)/n_{e,0}\right]^\Gamma.
\label{eq:Pe_polybeta}
\end{equation}
Here, $\Gamma$ is the polytropic index.

Polytropes are common in stellar astrophysics, and are used as a simple equation of state.  
Notably, $\Gamma = 1$ implies isothermality, $\Gamma=5/3$ describes adiabatic, non-relativistic gas, 
and $\Gamma = 4/3$ describes a relativistic gas.  For clusters, X-ray astronomers have typically found
that $\Gamma=$1.07--1.3 relates pressure to density outside the core, where the decline in temperature
begins between $r_c$ and $\sim 0.2 r_{vir}$, where $r_{vir}$ is the virial radius 
\citep[see][]{markevitch1998,arnaud1999}.

For SZE data, the application of a polytropic equation of state is straightforward.  
One parameter remains $\Delta T_0$, while the slope, $\beta$, is steepened by the factor $\Gamma$.  
Therefore, we have
%
\begin{equation}
\Delta T(R) = \Delta T_0\, [1 + (R/r_c)^2]^{-3\Gamma\beta/2+1/2}.
\label{eq:y_polybeta_sky}
\end{equation}
%
Pressure is derived from this model with a slight modification to Eq.~\ref{eq:y_0}, 
\begin{equation}
\Delta T_0 = 2 P_{e,0} \sqrt{\pi} \, r_c \, \frac{\Gamma(3\Gamma\beta/2 -1/2)}{\Gamma(3\Gamma\beta/2)},
\label{eq:dT_0_poly}
\end{equation}
%
where the $\Gamma$ in the parentheses is the polytropic index, and that outside is the Eulerian $\Gamma$
function.  The temperature profile that follows from this is
\begin{equation}
T(r) = \frac{P_{e}(r)}{k_B \, n_{e}(r)} =\frac{P_{e,0}}{k_B \, n_{e,0}} \left[n_e(r)/n_{e,0}\right]^{\Gamma-1}.
\label{eq:polyT}
\end{equation}
The temperature thus declines with radius with slope $\Gamma-1$.  While we were able to demonstrate
that this added sufficient flexibility to fit mock SZE observations of galaxy clusters, the use of this profile was
abandoned in lieu of an empirical pressure profile, presented in \S \ref{genNFW_model}.


==> references.tex <==
\singlespace 
\begin{thebibliography}{}
\addcontentsline{toc}{chapter}{Bibliography}

\bibitem[{{Bonamente} {et~al.}(2007){Bonamente}, {Joy}, {LaRoque}, {Carlstrom},
  {Nagai}, \& {Marrone}}]{bonamente2007}
{Bonamente}, M., {Joy}, M., {LaRoque}, S., {Carlstrom}, J., {Nagai}, D., \&
  {Marrone}, D. 2007, ArXiv e-prints, 708

\bibitem[{{Bonamente} {et~al.}(2004){Bonamente}, {Joy}, {Carlstrom}, {Reese},
  \& {LaRoque}}]{bonamente2004}
{Bonamente}, M., {Joy}, M.~K., {Carlstrom}, J.~E., {Reese}, E.~D., \&
  {LaRoque}, S.~J. 2004, \apj, 614, 56

\bibitem[{{Bonamente} {et~al.}(2006){Bonamente}, {Joy}, {LaRoque}, {Carlstrom},
  {Reese}, \& {Dawson}}]{bonamente2006}
{Bonamente}, M., {Joy}, M.~K., {LaRoque}, S.~J., {Carlstrom}, J.~E., {Reese},
  E.~D., \& {Dawson}, K.~S. 2006, ApJ, 647, 25

\bibitem[{{Cavaliere} \& {Fusco-Femiano}(1976)}]{cavaliere1976}
{Cavaliere}, A. \& {Fusco-Femiano}, R. 1976, \aap, 49, 137

\bibitem[{{Cavaliere} \& {Fusco-Femiano}(1978)}]{cavaliere1978}
---. 1978, \aap, 70, 677

\bibitem[{{da Silva} {et~al.}(2004){da Silva}, {Kay}, {Liddle}, \&
  {Thomas}}]{dasilva2004}
{da Silva}, A.~C., {Kay}, S.~T., {Liddle}, A.~R., \& {Thomas}, P.~A. 2004,
  \mnras, 348, 1401

\bibitem[{{Ebeling} {et~al.}(2001){Ebeling}, {Edge}, \& {Henry}}]{ebeling2001}
{Ebeling}, H., {Edge}, A.~C., \& {Henry}, J.~P. 2001, \apj, 553, 668

\bibitem[{{Gilks} {et~al.}(1996){Gilks}, {Richardson}, \&
  {Spiegelhalter}}]{gilks1996}
{Gilks}, W.~R., {Richardson}, S., \& {Spiegelhalter}, D.~J. 1996, Markov Chain
  Monte Carlo in Practice (Chapman and Hall)

\bibitem[{{Hawkins} {et~al.}(2004){Hawkins}, {Woody}, {Wiitala}, {Fredsti}, \&
  {Rauch}}]{hawkins2004}
{Hawkins}, D.~W., {Woody}, D.~P., {Wiitala}, B., {Fredsti}, J., \& {Rauch},
  K.~P. 2004, in Presented at the Society of Photo-Optical Instrumentation
  Engineers (SPIE) Conference, Vol. 5498, Millimeter and Submillimeter
  Detectors for Astronomy II. Edited by Jonas Zmuidzinas, Wayne S. Holland and
  Stafford Withington Proceedings of the SPIE, Volume 5498, pp. 567-578
  (2004)., ed. C.~M. {Bradford}, P.~A.~R. {Ade}, J.~E. {Aguirre}, J.~J. {Bock},
  M.~{Dragovan}, L.~{Duband}, L.~{Earle}, J.~{Glenn}, H.~{Matsuhara}, B.~J.
  {Naylor}, H.~T. {Nguyen}, M.~{Yun}, \& J.~{Zmuidzinas}, 567--578

\bibitem[{{Kravtsov} {et~al.}(2005){Kravtsov}, {Nagai}, \&
  {Vikhlinin}}]{kravtsov2005}
{Kravtsov}, A.~V., {Nagai}, D., \& {Vikhlinin}, A.~A. 2005, \apj, 625, 588

\bibitem[{{LaRoque} {et~al.}(2006){LaRoque}, {Bonamente}, {Carlstrom}, {Joy},
  {Nagai}, {Reese}, \& {Dawson}}]{laroque2006}
{LaRoque}, S.~J., {Bonamente}, M., {Carlstrom}, J.~E., {Joy}, M.~K., {Nagai},
  D., {Reese}, E.~D., \& {Dawson}, K.~S. 2006, \apj, 652, 917

\bibitem[{{Maughan} {et~al.}(2008){Maughan}, {Jones}, {Forman}, \& {Van
  Speybroeck}}]{maughan2008}
{Maughan}, B.~J., {Jones}, C., {Forman}, W., \& {Van Speybroeck}, L. 2008,
  \apjs, 174, 117

\bibitem[{{Maughan} {et~al.}(2007){Maughan}, {Jones}, {Jones}, \& {Van
  Speybroeck}}]{maughan2007b}
{Maughan}, B.~J., {Jones}, C., {Jones}, L.~R., \& {Van Speybroeck}, L. 2007,
  \apj, 659, 1125

\bibitem[{{Muchovej} {et~al.}(2007){Muchovej}, {Mroczkowski}, {Carlstrom},
  {Cartwright}, {Greer}, {Hennessy}, {Loh}, {Pryke}, {Reddall}, {Runyan},
  {Sharp}, {Hawkins}, {Lamb}, {Woody}, {Joy}, {Leitch}, \&
  {Miller}}]{muchovej2007}
{Muchovej}, S., {Mroczkowski}, T., {Carlstrom}, J.~E., {Cartwright}, J.,
  {Greer}, C., {Hennessy}, R., {Loh}, M., {Pryke}, C., {Reddall}, B., {Runyan},
  M., {Sharp}, M., {Hawkins}, D., {Lamb}, J.~W., {Woody}, D., {Joy}, M.,
  {Leitch}, E.~M., \& {Miller}, A.~D. 2007, \apj, 663, 708

\bibitem[{{Nagai}(2006)}]{nagai2006}
{Nagai}, D. 2006, \apj, 650, 538

\bibitem[{{Nagai} {et~al.}(2007{\natexlab{a}}){Nagai}, {Kravtsov}, \&
  {Vikhlinin}}]{nagai2007b}
{Nagai}, D., {Kravtsov}, A.~V., \& {Vikhlinin}, A. 2007{\natexlab{a}}, \apj,
  668, 1

\bibitem[{{Nagai} {et~al.}(2007{\natexlab{b}}){Nagai}, {Vikhlinin}, \&
  {Kravtsov}}]{nagai2007}
{Nagai}, D., {Vikhlinin}, A., \& {Kravtsov}, A.~V. 2007{\natexlab{b}}, \apj,
  655, 98

\bibitem[{{Pratt} \& {Arnaud}(2002)}]{pratt2002}
{Pratt}, G.~W. \& {Arnaud}, M. 2002, \aap, 394, 375

\bibitem[{{Raftery} \& {Lewis}(1992)}]{raftery1992}
{Raftery}, A.~L. \& {Lewis}, S. 1992, in Bayesian Statistics IV, ed. J.~M.
  {Bernardo} \& M.~H. {DeGroot} (Oxford University Press), 763

\bibitem[{{Raymond} \& {Smith}(1977)}]{raymond1977}
{Raymond}, J.~C. \& {Smith}, B.~W. 1977, \apjs, 35, 419

\bibitem[{{Smith} {et~al.}(2001){Smith}, {Brickhouse}, {Liedahl}, \&
  {Raymond}}]{smith2001}
{Smith}, R.~K., {Brickhouse}, N.~S., {Liedahl}, D.~A., \& {Raymond}, J.~C.
  2001, \apjl, 556, L91

\bibitem[{{Struble} \& {Rood}(1999)}]{struble1999}
{Struble}, M.~F. \& {Rood}, H.~J. 1999, \apjs, 125, 35

\bibitem[{{Vikhlinin} {et~al.}(2006){Vikhlinin}, {Kravtsov}, {Forman}, {Jones},
  {Markevitch}, {Murray}, \& {Van Speybroeck}}]{vikhlinin2006}
{Vikhlinin}, A., {Kravtsov}, A., {Forman}, W., {Jones}, C., {Markevitch}, M.,
  {Murray}, S.~S., \& {Van Speybroeck}, L. 2006, \apj, 640, 691

\end{thebibliography}

